Recovering a Molecule's 3D Dynamics from Liquid-phase Electron Microscopy Movies

The dynamics of biomolecules are crucial for our understanding of their functioning in living systems. However, current 3D imaging techniques, such as cryogenic electron microscopy (cryo-EM), require freezing the sample, which limits the observation of their conformational changes in real time. The innovative liquid-phase electron microscopy (liquid-phase EM) technique allows molecules to be placed in the native liquid environment, providing a unique opportunity to observe their dynamics. In this paper, we propose TEMPOR, a Temporal Electron MicroscoPy Object Reconstruction algorithm for liquid-phase EM that leverages an implicit neural representation (INR) and a dynamical variational auto-encoder (DVAE) to recover time series of molecular structures. We demonstrate its advantages in recovering different motion dynamics from two simulated datasets, 7bcq and Cas9. To our knowledge, our work is the first attempt to directly recover 3D structures of a temporally-varying particle from liquid-phase EM movies. It provides a promising new approach for studying molecules' 3D dynamics in structural biology.

==> backup/old-text.tex <==


% \subsection{Liquid phase EM reconstruction}
% Compared with the dataset of cryo-EM, the dataset collected by liquid phase electron microscope has approximately only \(10^{3-4}\) noisy images, and the SNR is slightly higher than that of cryo-electron microscope single particle image. In addition, each image of the data observed by the liquid phase electron microscope corresponds to a different shooting time of the same protein, so heterogeneity and continuity are both important. 

% \subsection{Learning based electron microscopy reconstruction}
% Determining the 3D electron density volume of protein from the 2D images collected by the electron microscope is meanly to solve the unknown 3D volume given 2D projections with unknown poses. Under the premise of known poses and high signal-to-noise ratio (SNR), backprojection-based methods can easily solve the problem of volume reconstruction mathematically (Hertle, 1981). Existing methods and software packages can handle the homogeneous 3D reconstruction together with pose estimation problem very well without known poses for all projections. Software package RELION (Sheres, 2012) and cryoSPARC (Punjani, 2017) are widely used in homogeneous cryo-EM reconstruction. But for heterogeneous reconstruction, methods using neural network will show advantages. 

% Both homogeneous and heterogeneous 3D electron density volume reconstruction from 2D cryo-EM images to 3D protein structures can be solved by neural network. For heterogeneous volume estimation, cryoDRGN build a low dimensional manifold in latent space to represent heterogeneity of different volumes corresponding to each projection (Zhong, (2019); Zhong, (2021); Zhong, (2021)). The network structure of cryoDRGN consists of an encoder and a coordinate-based decoder, which can directly estimate the electron density in Fourier space from noisy input images. CryoDRGN (Zhong, (2021)) assumes the poses to be determined by a consensus reconstruction and perform well in giving precise results of protein structural heterogeneity. An \textit{ab initio}estimation method for both poses and 3D volumes was proposed in CryoDRGN-BNB (Zhong, (2019)) and cryoDRGN2 (Zhong, (2021)). CryoAI (Levy, 2022) solves the task of pose estimation with a neural network-based method, and share parameters with the encoder for volume estimation.

% Other generative model-based architectures have also been applied to solve the problem of 3D reconstruction of electron density for cryo-EM. GAN and diffusion model based architecture are applied in CryoGAN (Gupta, 2021) and Latent Space Diffusion Models in cryoDRGN (Kreis, 2022) respectively.

% \subsection{Neural network dynamic sequence generative model}


%-----------------------------------------------------------------------

% \section{Methods}

% In order to reconstruct 3D volume from images captured by liquid phase electron microscopy (LEM), we proposed a dynamic neural network-based method, liquidDRGN (Dynamic deep Reconstructing Generative Network)(Figure 2). It can perform unsupervised reconstruction of the continuously changing protein 3D structure from the 2D image collected by the liquid phase EM. Inspired by the work of cryoDRGN using encoder and coordinate-based decoder architecture based on the variational autoencoder (VAE) (Kingma \& Welling, 2013), we formulate a dynamic neural network architecture based on deep Kalman filter (DKF) (Krishnan \textit{et al}., 2015; Krishnan \textit{et al}., 2017) to capture the dynamic information of protein conformational changes and encode the structure features of protein into latent variables. Compared to the vanilla VAE model, coordinate-based decoder can provide us with intrinsic conformational features of the final 3D volume independent of translation and rotation of the volume during LEM imaging. The training method finally presented includes a dynamic generation process from 2D images to 3D volumes and a forward image formation process. 

% \subsection{Image formation model}
% To solve the inverse problem of recovering a sequence of 3D volumes with a sequence of 2D images captured by liquid EM, not only do we need the dynamic deep reconstructing generative network, but also the image generating model. The formation of one image \(X\) can be modeled as:
%\begin{equation}
%X(r_x, r_y)=g * \int_{\mathbb{R}} V(R^{T}\mathbf{r}+t)dr_{z} + noise  
%\end{equation}
%where \(V\) is the electron density representing the 3D volume, \(R\) is an unknown orientation of the volume and \(t\) is an unknown in-plane translation. \(g\) represents the point spread function for the microscope which is caused by electron diffraction. With the help of the \textit{Fourier slice theorem} (Bracewell (1956)), which states that the Fourier transform of the projection of a n-dimensional function \(f(r)\) on to an m-dimensional linear submanifold is equal to an m-dimensional slice of the n-dimensional Fourier transform through the parallel projection manifold, the image formation model can also be formulated in Fourier domain as:
% \begin{equation}
% \hat{X}(k_x, k_y)=\hat{g}S(t)\hat{V}(R^T(k_x, k_y, 0)^T) + \epsilon
% \end{equation}
% which is obviously much easier to solve. \(\hat{g}\) is the contrast transfer function (CTF) of the microscope, \(S(t)\) is a phase shift operator to centralize the image \(X\) to \(X^{\prime}\) by operating translation \(-t\) to \(X\) in the real space and \(\epsilon\) is Gaussian noise in Fourier domain.

%\subsection{Generating model}
%The framework of our 3D structure generative model is based on DKF and Deep Kalman smoother (DKS) (Krishnan \textit{et al}., 2017), which can be viewed as a VAE decoder with a temporal inference model of the latent variable \(\mathbf{z}\). So a coordinate-based VAE decoder is used to approximate the volume generating function, \(\hat{V}(k_x,k_y,k_z, \mathbf{z}):\mathbb{R}^{3+n}\to\mathbb{R}\), representing a n-dimensional manifold of protein conformation in the Fourier domain. In detail the coordinate-based VAE decoder can bi formulated as \(p_\theta(\hat{V}|k,\mathbf{z})\), where \(\theta\) are parameters of a multilayer perception (MLP), \(k\in\mathbb{R}^3\) represents the 3D Cartesian coordinate and \(\mathbf{z}\) is the latent variable in n-dimensional manifold. Given a sample of Gaussian distribution \(\mathbf{z}\),the decoder outputs 3D voxel value \(\hat{V}(k, \mathbf{z})\) that represents the electron density of volume \(\hat{V}_\mathbf{z}\) at spacial frequency \(k\) in Fourier space. In order to get a complete 3D volume of the observed protein, \(k\) needs to traverse the entire 3D space in Fourier domain. 

% Due to the topological constraints between the 3D spectrum of volume and the 2D spectrum of projection of the 3D volume by Fourier slice theorem, only the Cartesian coordinates of one 2D plane need to be traversed when training. Suppose we have already known the translation and rotation corresponding to an image, according to Image formation model we can formulate the generative model during training as: 
%\begin{equation}
%\log p (\hat{X}|R, t, \mathbf{z}) = \sum_{i} \log p_\theta(\hat{V}|R^{T}c_{0}^{(i)}, \mathbf{z}) 
%\end{equation}
%here \(c_0\) represents the discretized lattice modeling the fixed 2D \(x\)-\(y\) plane before been rotated by rotation \(R\) and \(i\) indexes over the Cartesian coordinates of \(c_0\).   

%To capture both high frequency information and low frequency information of 3D protein volume, we do sine and cosine positional encoding to \(k\) instead of directly supply it to decoder. 

%\subsection{Inference model}
%Our inference model can be viewed as a temporal inference model of the latent variable \(\mathbf{z}\), as we suppose the translation \(t\) and rotation \(R\) are already known or can be inferred by existing pose estimation methods used in cryo-EM. The temporal inference model contains a dynamic variational encoder (Figure 2b) \(q_\phi(\mathbf{z}_{1:T}|\hat{X}_{1:T})\) with the variational parameters \(\phi\) which aims to approximate posterior probability of each latent variable given a sequence of observations in continuous time where \(T\) represents the sequence length of input images. In more detail, the input image sequence will be put into anMLP to extract \textit{pose-invariant} features of the protein’s structural heterogeneity and then into a bidirectional recurrent neural network (RNN) (Elman, 1990) that extracts temporal features from entire sequence of encoded features. At the same time, we use an Long Short-Term Memory (LSTM) (Hochreiter \& Schmidhuber, 1997) model \(p_{\theta_z}(\mathbf{z}_t|\mathbf{z}_t-1)\) to simulate the state transition process of the protein structure, so as to obtain the prior distribution of a serial of variables in the latent space.

% Given a sequence of images captured by liquid EM with each image represented as a flattened vector, the temporal encoder outputs a same-length sequence of latent variables. Each latent variable can be viewed as a multivariate Gaussian distribution with mean and diagonal standard deviation inferred by the dynamic variational encoder. The entire latent variable sequence aims to parameterize posterior probability \(p(\mathbf{z}_{1:T}|\hat{X}_{1:T})\), and prior probability is given by the state transition function modeled by LSTM. Note that prior probability of the first latent variable in one sequence is a standard normal, following the DKS Framework.

%\subsection{Reconstruction pipeline}
%Given an image sequence captured by liquid EM, we hope to reconstruct the specific 3D volume of the protein at different shooting times, the problem can be expressed as \(\hat{V}_{1:T} = \hat{V}_{1:T}(\hat{X}_{1:T})\). Typically the problem can be transformed intofinding a \textit{maximum a posterior} estimate of \(\hat{V}_{1:T}\) given observations 
%\(\hat{X}_{1:T}\):
%\begin{equation}
%    \hat{V}_{1:T} = \underset{\hat{V}_{1:T}}{\arg \max} \log p(\hat{X}_{1:T}|\hat{V}_{1:T}) + 
%    \log p(\hat{V}_{1:T})
%\end{equation}
%In particular, we hope to reconstruct a 3D conformation for each captured image to represent the protein volume at that capturing time. Therefore, for each shot we reconstruct one volume \(\hat{V}_t\). Following the DKS framework, the posterior probability is approximated as a temporalencoder-decoder architecture as:
%\begin{equation}
%    p(\hat{V}_{1:T}|\hat{X}_{1:T}) = \prod_{t=1}^{T} p_\theta(\hat{V}_{t}|\mathbf{z}_{t})  %q_\phi(\mathbf{z}_{t}|\hat{X}_{1:T})
%\end{equation}
%where \(p_\theta\) represents the inference model and \(q_\phi\) represents the generating model. The objective function is the Evidence Low Bound (ELBO):
%\begin{equation}
%\begin{aligned}
%\mathcal{L}(\hat{X}_{i_{1:T}};\phi,\theta)=\sum_{t=1}^{T}\mathbb{E}_{q_{\phi}(\mathbf{z}_{t}|\hat{X}_{i_{1:T}})}[\log p_\theta(\hat{X}_{i_{t}}|\mathbf{z}_{t})]\\
%-D_{KL}(q_{\phi}(\mathbf{z}_{t}|\hat{X}_{i_{1:T}})|p_{\theta_{z}}(\mathbf{z}_t|\mathbf{z}_{t-1}))\\
%\end{aligned}
%\end{equation}
%Generation loss term gives the similarity of input images with generated images projected by image formation model and KL divergence term evaluates the similarity between the generated value of latent variables and the predicted results of the state transition process, constrains the relationship between the latent variables of the frames before and after the sequence generation model, which reflects the molecular dynamics information of the protein conformation heterogeneity. 

% For each independent liquid phase EM dataset, we need to do separate training to learn the structural information of the protein and the timing information during the conformational change process. We both consider using liquidDRGN for training from scratch and using cryoDRGN for pre-training, then using liquidDRGN for fine-tuning for several epochs. The reconstruction results show that the pre-training method can better learn the protein 3D volume heterogeneity represented by the manifold in the latent space and provide a reference number of training epochs. At the same time, the pose estimation method provided by cryoDRGN can also be appropriately used while training. 


%-----------------------------------------------------------------------

% \section{Results}

%-----------------------------------------------------------------------

